Numerical Study of Nearly Singular Solutions of the 3-D Incompressible Euler Equations

In this paper, we perform a careful numerical study of nearly singular solutions of the 3D incompressible Euler equations with smooth initial data. We consider the interaction of two perturbed antiparallel vortex tubes which was previously investigated by Kerr in \cite{Kerr93,Kerr05}. In our numerical study, we use both the pseudo-spectral method with the 2/3 dealiasing rule and the pseudo-spectral method with a high order Fourier smoothing. Moreover, we perform a careful resolution study with grid points as large as $1536\times1024\times 3072$ to demonstrate the convergence of both numerical methods. Our computational results show that the maximum vorticity does not grow faster than doubly exponential in time while the velocity field remains bounded up to T=19, beyond the singularity time $T=18.7$ reported by Kerr in \cite{Kerr93,Kerr05}. The local geometric regularity of vortex lines near the region of maximum vorticity seems to play an important role in depleting the nonlinear vortex stretching dynamically.

==> Makefile <==

ifeq (x$(target), x) then
  TARGET=euler_comput
else
  TARGET=$(target)
endif

default : 
	@echo run \"make dvi\" to get DVI file
	@echo run \"make ps\"\  to get PS file
	@echo run \"make pdf\" to get PDF file

dvi : 
	latex $(TARGET).tex
	bibtex $(TARGET)
	latex $(TARGET).tex

ps : dvi
	dvips -o $(TARGET).ps $(TARGET).dvi

pdf : dvi
	dvipdf $(TARGET).dvi $(TARGET).pdf

.PHONY : dvi ps pdf


